Pro or Anti? A Social Influence Model of Online Stance Flipping

Social influence characterizes the change of an individual's stances in a complex social environment towards a topic. Two factors often govern the influence of stances in an online social network: endogenous influences driven by an individual's innate beliefs through the agent's past stances and exogenous influences formed by social network influence between users. Both endogenous and exogenous influences offer important cues to user susceptibility, thereby enhancing the predictive performance on stance changes or flipping. In this work, we propose a stance flipping prediction problem to identify Twitter agents that are susceptible to stance flipping towards the coronavirus vaccine (i.e., from pro-vaccine to anti-vaccine). Specifically, we design a social influence model where each agent has some fixed innate stance and a conviction of the stance that reflects the resistance to change; agents influence each other through the social network structure.From data collected between April 2020 to May 2021, our model achieves 86\% accuracy in predicting agents that flip stances. Further analysis identifies that agents that flip stances have significantly more neighbors engaging in collective expression of the opposite stance, and 53.7% of the agents that flip stances are bots and bot agents require lesser social influence to flip stances.

==> tables/notations.tex <==
\begin{table*}[!ht]
\begin{center}
\begin{tabular}{|p{2.5cm}|p{14cm}|}
\hline
%\textbf{Notation} & \textbf{Importance} \\ \hline
$Y$ \newline ($Y_{agent}$, $Y_{neighbor}$) & the stance towards vaccination, i.e. pro- or anti-vaccination (stance of agent in focus, stance of neighbor) \\ \hline 
$X$ ($X_*$) & endogeneous and exogeneous variables (observable variables) \\ \hline 
$B$ ($B_*$) & coefficients of effects of variables $X$ (coefficients of effects of observable variables $X_*$) \\ \hline
$I$ & Agent's influence stance score \\ \hline 
$D$ & Deflection score between agent's stance and influence from variables \\ \hline
$\gamma$ & Agent's stance strength \\ \hline
$R$ & Reciprocity between two agents \\ \hline 
\end{tabular}
\caption{Notation Summary}
\label{tab:notations}
\end{center}
\end{table*}
